From Code to Courtroom: LLMs as the New Software Judges

Recently, Large Language Models (LLMs) have been increasingly used to automate SE tasks such as code generation and summarization. However, evaluating the quality of LLM-generated software artifacts remains challenging. Human evaluation, while effective, is very costly and time-consuming. Traditional automated metrics like BLEU rely on high-quality references and struggle to capture nuanced aspects of software quality, such as readability and usefulness. In response, the LLM-as-a-Judge paradigm, which employs LLMs for automated evaluation, has emerged. Given that LLMs are typically trained to align with human judgment and possess strong coding abilities and reasoning skills, they hold promise as cost-effective and scalable surrogates for human evaluators. Nevertheless, LLM-as-a-Judge research in the SE community is still in its early stages, with many breakthroughs needed. This forward-looking SE 2030 paper aims to steer the research community toward advancing LLM-as-a-Judge for evaluating LLMgenerated software artifacts, while also sharing potential research paths to achieve this goal. We provide a literature review of existing SE studies on LLM-as-a-Judge and envision these frameworks as reliable, robust, and scalable human surrogates capable of evaluating software artifacts with consistent, multi-faceted assessments by 2030 and beyond. To validate this vision, we analyze the limitations of current studies, identify key research gaps, and outline a detailed roadmap to guide future developments of LLM-as-a-Judge in software engineering. While not intended to be a definitive guide, our work aims to foster further research and adoption of LLM-as-a-Judge frameworks within the SE community, ultimately improving the effectiveness and scalability of software artifact evaluation methods.

==> sections/04_vision.tex <==
\section{Limitations}
\label{sec:limitations}


Limitations:




1. Lack of high-quality and large-scale human-annotated benchmarks



In Section \ref{sec:review}, we review numerous works that investigate the effectiveness of LLM-as-a-Judge in SE. When evaluating \toolname for corrections code generations, we can utilize the existing benchmarks, such as HumanEval, and MBPP.
However, when evaluating the alignment of human judgment in more nuanced analysis, such as helpfulness readability, a significant limitation of these current works is the small-scale experiments~\cite{wang2025can, wu2024can, ahmad2024can}, usually just a few hundred samples. 
For example, Want et al.~\cite{wang2025can} conduct experiments on three SE tasks, including Code Translation, Code Generation, and Code Summarization, in a total of 450 samples. 
420 samples are used by Ahmed et al.~\cite{ahmad2024can} in code summariztion evaluation. 
Despite the small scale may still be sufficient to demonstrate statistical significance, it is still important to have a larger scale to ensure the generalizability and reliability of the findings.




Numerous works also conclude with different findings. However, as the experiments are usually conducted on different datasets, it is difficult to draw a conclusion.

For example, Wang et al.~\cite{wang2025can} find that \toolname methods are completely defeated by conventional metrics (i.e., ROUGE~\cite{lin2004rouge}, METEOR~\cite{banerjee2005meteor}, and ChrF++~\cite{popovic2017chrf++}) in code summarization in human alignment, while Wu et al.~\cite{wu2024can} find that their proposed method, CODERPE, surpasses traditional metrics in achieving the best performance for code summarization. 
The difference in findings can be attributed to multiple factors, such as the prompt design and the selection of an appropriate LLM.
Therefore, as the first step, we believe it is important to develop comprehensive and diverse benchmarks that facilitate a holistic evaluation of \toolname in SE.







* LLM-as-a-judge cannot perform well on challenging benchmarks, such as bigcodebench and 
